Towards Practicality of Sketch-Based Visual Understanding

Sketches have been used to conceptualise and depict visual objects from pre-historic times. Sketch research has flourished in the past decade, particularly with the proliferation of touchscreen devices. Much of the utilisation of sketch has been anchored around the fact that it can be used to delineate visual concepts universally irrespective of age, race, language, or demography. The fine-grained interactive nature of sketches facilitates the application of sketches to various visual understanding tasks, like image retrieval, image-generation or editing, segmentation, 3D-shape modelling etc. However, sketches are highly abstract and subjective based on the perception of individuals. Although most agree that sketches provide fine-grained control to the user to depict a visual object, many consider sketching a tedious process due to their limited sketching skills compared to other query/support modalities like text/tags. Furthermore, collecting fine-grained sketch-photo association is a significant bottleneck to commercialising sketch applications. Therefore, this thesis aims to progress sketch-based visual understanding towards more practicality.

==> authors_publication.tex <==
\chapter{Appendix A: Author's Publications}
 \label{chapter:Publication}
     \vspace{-2em}
 During my PhD, I have published these papers, of which the first five mentioned here contribute to this thesis. 
    
 \begin{enumerate}
   \item  \noindent \textbf{Ayan Kumar Bhunia}, Yongxin Yang, Timothy M. Hospedalis, Tao Xiang, Yi-Zhe Song.``Sketch Less for More: On-the-Fly Fine-Grained Sketch Based Image Retrieval". IEEE Conference on Computer Vision and Pattern Recognition (\textbf{CVPR}) 2020. [\textbf{Oral}]

    
   \item \noindent \textbf{Ayan Kumar Bhunia}, Pinaki Nath Chowdhury, Yongxin Yang, Timothy Hospedales, Tao Xiang, Yi-Zhe Song. ``Vectorization and Rasterization: Self-Supervised Learning for Sketch and Handwriting". 
    IEEE Conference on Computer Vision and Pattern Recognition (\textbf{CVPR}) 2021. 
    

    \item \noindent \textbf{Ayan Kumar Bhunia}, Pinaki Nath Chowdhury, Aneeshan Sain, Yongxin Yang, Tao Xiang, Yi-Zhe Song. ``More Photos are All You Need: Semi-Supervised Learning for Fine-Grained Sketch Based Image Retrieval".  
    IEEE Conference on Computer Vision and Pattern Recognition (\textbf{CVPR}) 2021. 

    
   \item \noindent \textbf{Ayan Kumar Bhunia}, Viswanatha Reddy Gajjala, Subhadeep Koley, Rohit Kundu, Aneeshan Sain, Tao Xiang, Yi-Zhe Song. ``Doodle It Yourself: Class Incremental Learning by Drawing a Few Sketches".  
    IEEE Conference on Computer Vision and Pattern Recognition (\textbf{CVPR}) 2022. 

    
   \item \noindent \textbf{Ayan Kumar Bhunia}, Subhadeep Koley, Abdullah Faiz Ur Rahman Khilji, Aneeshan Sain, Pinaki Nath Chowdhury, Tao Xiang, Yi-Zhe Song. ``Sketching without Worrying: Noise-Tolerant Sketch-Based Image Retrieval".  
    IEEE Conference on Computer Vision and Pattern Recognition (\textbf{CVPR}) 2022.  
    
    
\item \noindent \textbf{Ayan Kumar Bhunia*}, Ayan Das*, Umar Riaz Muhammad*, Yongxin Yang, Timothy M. Hospedalis, Tao Xiang, Yulia Gryaditskaya, Yi-Zhe Song. ``Pixelor: A Competitive Sketching AI Agent. So you think you can beat me?".  
    \textbf{SIGGRAPH Asia} 2020.

\item \noindent Aneeshan Sain, \textbf{Ayan Kumar Bhunia}, Yongxin Yang, Tao Xiang, Yi-Zhe Song. ``Cross-Modal Hierarchical Modelling for Fine-Grained Sketch Based Image Retrieval".  
    British Machine Vision Conference (\textbf{BMVC}) 2020.

\item \noindent Ruoyi Du, Dongliang Chang, \textbf{Ayan Kumar Bhunia}, Jiyang Xie, Zhanyu Ma, Yi-Zhe Song, Jun Guo. ``Fine-grained visual classification via progressive multi-granularity training of jigsaw patches".  
    European Conference on Computer Vision (\textbf{ECCV}) 2020.
    
\item \noindent Aneeshan Sain, \textbf{Ayan Kumar Bhunia}, Yongxin Yang and , Tao Xiang, Yi-Zhe Song. ``StyleMeUp: Towards Style-Agnostic Sketch-Based Image Retrieval".  
    IEEE Conference on Computer Vision and Pattern Recognition (\textbf{CVPR}) 2021.

\item \noindent \textbf{Ayan Kumar Bhunia}, Shuvozit Ghose, Amandeep Kumar, Pinaki Nath Chowdhury, Aneeshan Sain, Yi-Zhe Song. ``MetaHTR: Towards Writer-Adaptive Handwritten Text Recognition".  
    IEEE Conference on Computer Vision and Pattern Recognition (\textbf{CVPR}) 2021.
    
    \item \noindent \textbf{Ayan Kumar Bhunia}, Aneeshan Sain, Pinaki Nath Chowdhury, Yi-Zhe Song. ``Text is Text, No Matter What: Unifying Text Recognition using Knowledge Distillation".  
    IEEE International Conference on Computer Vision (\textbf{ICCV}) 2021.

\item \noindent \textbf{Ayan Kumar Bhunia}, Pinaki Nath Chowdhury, Aneeshan Sain, Yi-Zhe Song. ``Towards the Unseen: Iterative Text Recognition by Distilling from Errors".  
    IEEE International Conference on Computer Vision (\textbf{ICCV}) 2021.

\item \noindent \textbf{Ayan Kumar Bhunia}, Aneeshan Sain, Amandeep Kumar, Shuvozit Ghose, Pinaki Nath Chowdhury, Yi-Zhe Song. ``Joint Visual Semantic Reasoning: Multi-Stage Decoder for Text Recognition". IEEE International Conference on Computer Vision (\textbf{ICCV}) 2021.

\item \noindent Pinaki Nath Chowdhury, \textbf{Ayan Kumar Bhunia}, Viswanatha Reddy Gajjala, Aneeshan Sain, Tao Xiang, Yi-Zhe Song. ``Partially Does It: Towards Scene-Level FG-SBIR with Partial Input". 
	IEEE Conference on Computer Vision and Pattern Recognition(\textbf{CVPR}) 2022. 

 \item \noindent Aneeshan Sain, \textbf{Ayan Kumar Bhunia}, Vaishnav Potlapalli , Pinaki Nath Chowdhury, Tao Xiang, Yi-Zhe Song. ``Sketch3T: Test-time Training for Zero-Shot SBIR".  
    IEEE Conference on Computer Vision and Pattern Recognition (\textbf{CVPR}) 2022.

    
\item \noindent \textbf{Ayan Kumar Bhunia}, Aneeshan Sain, Parth Hiren Shah, Animesh Gupta, Pinaki Nath Chowdhury, Tao Xiang , Yi-Zhe Song. ``Adaptive Fine-Grained Sketch-Based Image Retrieval".  
    European Conference on Computer Vision (\textbf{ECCV}) 2022.  

\item \noindent Pinaki Nath Chowdhury, Aneeshan Sain, \textbf{Ayan Kumar Bhunia},  Tao Xiang, Yulia Gryaditskaya,  Yi-Zhe Song . ``FS-COCO: Towards Understanding of Freehand Sketches of Common Objects in Context".  
    European Conference on Computer Vision (\textbf{ECCV}) 2022.  

\end{enumerate}
